Robust Identifiability in Linear Structural Equation Models of Causal Inference

In this work, we consider the problem of robust parameter estimation from observational data in the context of linear structural equation models (LSEMs). LSEMs are a popular and well-studied class of models for inferring causality in the natural and social sciences. One of the main problems related to LSEMs is to recover the model parameters from the observational data. Under various conditions on LSEMs and the model parameters the prior work provides efficient algorithms to recover the parameters. However, these results are often about generic identifiability. In practice, generic identifiability is not sufficient and we need robust identifiability: small changes in the observational data should not affect the parameters by a huge amount. Robust identifiability has received far less attention and remains poorly understood. Sankararaman et al. (2019) recently provided a set of sufficient conditions on parameters under which robust identifiability is feasible. However, a limitation of their work is that their results only apply to a small sub-class of LSEMs, called ``bow-free paths.'' In this work, we significantly extend their work along multiple dimensions. First, for a large and well-studied class of LSEMs, namely ``bow free'' models, we provide a sufficient condition on model parameters under which robust identifiability holds, thereby removing the restriction of paths required by prior work. We then show that this sufficient condition holds with high probability which implies that for a large set of parameters robust identifiability holds and that for such parameters, existing algorithms already achieve robust identifiability. Finally, we validate our results on both simulated and real-world datasets.

==> proofReduction.tex <==
\section{Missing Proofs in Section~\ref{sec:reduction}}

\reduction*

	Before we prove the theorem, we state the following observation about bow-free models of $\LSEM$. 
		\begin{observation}[\cite{Tian2002}]
			\label{obs:topSort}
			Let $G = (U, E, F)$ be a given bow-free $\LSEM$ causal model. Let $L$ denote the length of the longest directed path using edges in $E$. Then there exists an ordering of vertices $\{ V_{\sigma(i)} \}_{i \in [L]}$ such that every edge $e = (u, v) \in E$ has the orientation $u \in V_{\sigma(i)}$ and $v \in V_{\sigma(j)}$ with $j > i$.
		\end{observation}
		
	
\begin{proof}
	Consider the graph $G$ and let $\sigma$ denote the topological sort order of the directed graph. Let $V_{\sigma(1)} \curlyeqprec  V_{\sigma(2)} \curlyeqprec \ldots \curlyeqprec V_{\sigma(L)}$ denote the vertices that have an order $\sigma(1), \sigma(2), \ldots \sigma(L)$ respectively. Let $\mySigma$ denote the covariance matrix of the data corresponding to this graph.
	
		In the proof outline, we described a simple method that introduced twice the number of required nodes and increased the number of layers by a factor of $2$. Here, we show a careful reduction that introduces lesser nodes and retains the number of layers to be the length of maximum directed path in the graph $G$. The reduction is formally defined in Construction~\ref{cons:reduction}.
		
		We first describe a gadget that will be used in our reduction.
		\begin{gadget}[$(q, r)$-directed path gadget]
			\label{gad:replaceLengthOne}
			Consider a directed edge $u \rightarrow v$ in the graph $G$. Let $(q, r)$ be given input parameters. The $(q, r)$-directed path gadget consists of vertices $u, v$ along with set of vertices $R_1, R_2, \ldots, R_q$ such that $|R_i|=r$ for $i \neq q$ and $|R_q| = r^2$. Let $r_{i, j}$ denote the $i^{th}$ vertex in the set $R_j$. Finally, we add a new vertex denoted by $w_0$. Thus, the new set of vertices is the set $\{u, v, w_0\} \cup R_1 \cup R_2 \cup \ldots \cup R_q$.
			
			For every vertex $r_{i, 1} \in R_1$, we have edges $u \rightarrow r_{i, 1}$ with weight forced to be $\frac{1}{r}$. For layers $R_2, R_3, \ldots, R_q$ we have the following incoming directed edges. For a given vertex $r_{i, j}$ we add a single incoming directed edge from $r_{i', j-1}$ into $r_{i, j}$ for every $i' \in [r]$, with the weights on all these edges forced to $\frac{1}{r}$. We add directed edge from every vertex $r_{i, q} \in R_q$ to $w_0$. Once again we force the edge weight of these edges to be $\frac{1}{r}$. Finally, we add an edge from $w_0$ to $v$. We do not impose any constraint on the weights of this edge.
		\end{gadget}
		Given a $(q, r)$-directed path gadget for a directed edge $(u \rightarrow v)$ we call $u$ to be the \emph{head}, $w_0$ to be \emph{collector} and $v$ to be the \emph{tail} of the gadget.
		
	\begin{construction}[Construction of the new graph]
		\label{cons:reduction}
		Consider an edge that goes from vertex $v_s \in V_{\sigma(i)}$ to another vertex $v_t \in V_{\sigma(j)}$ such that $j-i \geq 2$. Let $r$ be a parameter that will be fixed later in the analysis. We introduce $(j-i-1)*r$ new nodes, denoted by layers $U_1, U_2, \ldots, U_{j-i-1}$ with $|U_a| = r$. We replace the directed edge $v_s \rightarrow v_t$ with a $(j-i-1, r)$-directed path gadget described in Gadget~\ref{gad:replaceLengthOne}. Let $\cF_{v_s, v_t}$ denote the set of bidirected edges incident on either $v_s$ or $v_t$. For every bidirected edge $f \in \cF_{v_s, v_t}$ where $f=(w, v)$ with $v \in \{ v_s, v_t\}$, we introduce a bidirected edge $(w_0, w)$ into $G'$. We do this for every $(q, r)$-directed path gadget introduced. We retain all directed and bidirected edges of $G$ in $G'$. We repeatedly do this for every directed edge  that goes across \emph{layers} in a topological ordering in the DAG. 

		% We add dummy vertices (no incoming and outgoing directed or bidirected edges) in any layer to ensure that each layer has the same number of vertices.

		%we introduce bidirected edges $(U_1, w), (U_2, w), \ldots, (U_{j-i-1}, w)$ into the model. Here $(U_i, w)$ denotes that a bidirected edge is added between every vertex of $u_i \in U_i$ and $w$. Likewise, for every bidirected edge $f \in \cF_{v_s, v_t}$ where $f=(w, v)$ with $v \in \{ v_s, v_t\}$, 
			\end{construction}
	
	Let $G'$ be the graph that is obtained after applying Construction~\ref{cons:reduction} to $G$. Let $\mySigma'$ denote the corresponding data covariance matrix corresponding to this graph. Construction~\ref{cons:Sigma} describes how to construct $\mySigma'$ formally.
	\begin{construction}[Construction of new covariance matrix]
		\label{cons:Sigma}
		For every entry $(u, v)$ such that $u \in G$ and $v \in G$, we let $\mySigma'(u, v) = \mySigma(u, v)$. Consider an entry $(u, v)$ such that $u \in G$ while $ v\ not \in G$. Let $w$ denote the head of $v$ in a $(q, r)$ gadget used in Construction~\ref{cons:reduction}. Then we let $\mySigma'(u, v) = \frac{1}{r} \mySigma(u, w)$. Finally, consider an entry $(u, v)$ such that $u \not \in G$ and $v \not \in G$. Let $w_1, w_2$ denote the head of $u$ and $v$ respectively, in a $(q, r)$ gadget used in Construction~\ref{cons:reduction}. Then we let $\mySigma'(u, v) = \frac{1}{r^2} \mySigma(w_1, w_2)$.
	\end{construction}
	
	\xhdr{$G'$ satisfies \emph{bow-free} and \emph{layered} properties.}
	First, we argue that the new graph satisfies the bow-free property. Consider any pair of directed and bidirected edge in $G'$. From Construction~\ref{cons:reduction} we ensure that we never add a bidirected edge between any pair of vertices both of which do not exist in $G$. In particular, all new bidirected edges go from a collector of some gadget to a vertex $w \in G$ such that $w$ is not the tail of the same gadget. Thus, there is a path of length at least $2$ between the collector and $w$ and thus, remains bow-free. It is easy to see that the reduction creates layers such that a directed edge goes only from one layer to the next, since edges that skip layers are replaced by a $(q, r)$-directed path gadget that replaces this edge with a path with edges going across one layer to its neighboring layer.
	
	\xhdr{$\mySigma'$ respects $\LSEM$ equations in $G$.}
	We will now show that the construction of $\mySigma'$ in Construction~\ref{cons:Sigma} implies that it respects the same set of $\LSEM$ equations as that of $G$. In particular, consider a directed edge $(u \rightarrow v) \in G$ and let $X_u$ and $X_v$ denote the corresponding random variables. Let the $\LSEM$ equation in the original graph be,
		\begin{equation}
			\label{eq:reductionOriginal}	
			X_v = X_u + \eta_v.
		\end{equation}

		Now consider the graph $G'$. Let $X_{U_1}, X_{U_2}, \ldots, X_{U_r}, X_{w_0}$ denote the newly introduced random variables. It is easy to verify that the following system of equations is equivalent to Eq.~\eqref{eq:reductionOriginal}.
		\begin{align}
			X_{U_i} &= \frac{1}{r} X_u \qquad	\forall i \in [q] \nonumber \\
			X_{w_0} &= \sum_{z \in U_q} \frac{1}{r} X_z  \nonumber \\
			X_v &= X_{w_0} + \eta_v. \label{eq:reductionNew}
		\end{align}
		Consider the matrix $\mathbb{E}[\vec{X}^T \cdot \vec{X}]$ obtained by the system Eq.~\eqref{eq:reductionNew}. We can verify that this corresponds to the $\mySigma'$ described in Construction~\ref{cons:Sigma}.
		
		\xhdr{Algorithm in \cite{FDD2012Annals} solves the same set of equations for $G'$ as in $G$.}
		We will now show that applying the algorithm in \cite{FDD2012Annals} implies that it will solve the same set of linear equations for the reduced instance as in the original instance. Let $(u, w_0, v)$ be any head, collector and tail tuple for some gadget. The above will imply that the edge weight of $(w_0, v)$ in $G'$ will be the same as that of $(u, v)$ in $G$.
		
		Let $P_{v} = \{ p_1, p_2, \ldots, p_d\}$ denote the set of parents of $v$ in $G$. From the construction we have the following observation.
		\begin{observation}
			\label{obs:incomingEdges}
			If $v_i$ is a vertex in $G'$ that is also a vertex in $G$ then none of the incoming edges into $v_i$ has a weight that is \emph{forced}.
		\end{observation}
		
		Let $Y_v$ denote the set of vertices corresponding to $v$ that satisfies the half-trek criterion and required by the algorithm in \cite{FDD2012Annals} as input. The construction ensures that $Y_{v}$ continues to remain a set of vertices that can be reached from $v$ via a half-trek. This is because there exists a half-trek from $v$ to $Y_v$ in $G$, and the edges are only added and never removed. Moreover, from Observation~\ref{obs:incomingEdges} we note that the incoming edges into vertices that are present in both $G$ and $G'$ do not have those with forced edge weights. Thus, we have for every $w \in Y_{v}$,  $\myLambda_{(pa(w), \{w\})}' = \myLambda_{(pa(w), \{w\})}$. Moreover, from Construction~\ref{cons:Sigma} we see that in row corresponding to $pa(w)$, the entries $(i, w)$ where $i \in G$ in $\mySigma'$ is the same as that in $\mySigma$. Thus, from the description of the algorithm in Definition~\ref{def:FDDAlg}, the algorithm solves for the same set of linear equations corresponding to $(G', \mySigma')$ as that in $(G, \mySigma)$.

		\xhdr{Putting it together.}
		Set $r = \sqrt{n}$. Note that some of the edge-weights are already fixed and thus, we need to ensure that the sub-graph of $G'$ induced by the edges not already determined satisfy \ref{cons:reduction}-\ref{cons:Sigma}. Thus, as long as this is satisfied, our reduction implies that the condition number theorem~\ref{thm:MainTheorem} extends to arbitrary bow-free graphs.
\end{proof}

\xhdr{Discussion.} The proof of Theorem~\ref{thm:reduction} has some subtleties, which we would like to point out here. The algorithm in \cite{FDD2012Annals} as described in Definition~\ref{def:FDDAlg} performs parameter estimation, layer-by-layer. This helps us with proving Theorem~\ref{thm:MainTheorem} and Theorem~\ref{thm:random}. However, as stated originally it takes as input, the matrix $\mySigma$, the weight matrix $\myLambda$ for the previous layers and a vertex $v$ in the current layer, and estimates the weight of all incoming edges into $v$. In particular, we give as input all edges whose weights are already \emph{forced} directly as input to the algorithm. Thus, using the reduction, we can reuse the main condition number result in Theorem~\ref{thm:MainTheorem} by appropriately modifying the definitions of the layers $V_I$. In particular, we look at the graph restricted to all \emph{unforced} edges. We compute the topological sort order of this graph. We let $V_I$ to be the set of all vertices whose order is $I$. Then, it can be verified that the proof of Theorem~\ref{thm:MainTheorem} goes through.


==> reductionToLayeredGraphs.tex <==
\section{Inverse Problems on General Bow-free DAGs}
\label{sec:reduction}
In this section, we show that computing the inverse problem on general \emph{bow-free} causal DAGs can be reduced to the problem of finding inverse maps on an appropriate $k$-layered bow-free causal DAGs. Thus, it suffices to show stability results for layered DAGs. Formally, consider a causal graph structure $G = (V, E, F)$ such that the directed edges $E$ form a directed acyclic graph and the bidirected edges $F$ form a bow-free structure. Recall that the goal is to compute the map in Eq.~\eqref{eq:inverseProblem}. We will argue that there exists a $k$-layered bow-free causal graph $G'=(V', E', F')$ and a corresponding data covariance matrix $\mySigma'$ such that the inverse map,
	\begin{equation}
		\label{eq:inverseProblemK}
			\Psi_{G'}^{-1}: \mySigma' \rightarrow \myLambda',
	\end{equation}
	can be used to compute the map in Eq.~\eqref{eq:inverseProblem}. Formally, we prove the following theorem. 
	
	\begin{figure}
	\centering
	\includegraphics[scale=0.4]{Figures/ReductionExample}
	\caption{$1^{st}$: Non-layered. $2^{nd}$: Layered bow-free. $3^{rd}$: gadget to replace weight $1$ edge.}
	\label{fig:reduction}
\end{figure}

	

\begin{restatable}{theorem}{reduction}
	\label{thm:reduction}
	Consider a bow-free causal graph $G=(V, E, F)$ and a data covariance matrix $\mySigma \in \mathbb{R}^{n \times n}$. There exists a \emph{$k$-layered} bow-free causal DAG $G'=(V', E', F')$ with $n' := |V'|$ and a corresponding data covariance matrix $\mySigma' \in \mathbb{R}^{n' \times n'}$ such that the inverse map $\Psi_{G'}^{-1}(\mySigma')$ can be used to uniquely recover the inverse map $\Psi_{G}^{-1}(\mySigma)$ as defined in Equations~\eqref{eq:inverseProblem} and \eqref{eq:inverseProblemK} respectively. Additionally, graph $G'$ satisfies $k \leq n^2$ and $n' \leq n^6$.
\end{restatable}

\xhdr{Proof Outline.} The key idea is to split an edge that goes across many layers into multiple edges such that the product of edge-weights remain the same as the original edge. Moreover, we ensure that the noise variables are appropriately correlated for the newly added vertices.  Figure~\ref{fig:reduction} gives an illustration of the reduction on a $4$-node graph where the edge $(v_1, v_4)$ is replaced by a path $v_! \rightarrow u_1 \rightarrow u_2 \rightarrow v_4$ with appropriate noise correlations. Moreover, the edge weights of $(v_1, u_1)$ and $(u_1, u_2)$ is forced to be $1$. To ensure it satisfies the Assumptions in Model~\ref{mod:mainModel}, we replace any edge with weight $1$ with a gadget (in Fig.~\ref{fig:reduction}) each with weight $1/k$. Thus the algorithm in \citet{FDD2012Annals} will recover the weight of $(u_2, v_4)$ to be the same as the weight in $(v_1, v_4)$ in the original model. Our reduction implies that the algorithm in \citet{FDD2012Annals} will solve the \emph{exact} same set of equations in the new graph as in the old graph. Thus, this reduction preserves condition number bounds and generic identifiability property.

